Limitations on Observability of Effects in Cyber-Physical Systems

Increased interconnectivity of Cyber-Physical Systems, by design or otherwise, increases the cyber attack surface and attack vectors. Observing the effects of these attacks is helpful in detecting them. In this paper, we show that many attacks on such systems result in a control loop effect we term Process Model Inconsistency (PMI). Our formal approach elucidates the relationships among incompleteness, incorrectness, safety, and inconsistency of process models. We show that incomplete process models lead to inconsistency. Surprisingly, inconsistency may arise even in complete and correct models. We illustrate our approach through an Automated Teller Machine (ATM) example, and describe the practical implications of the theoretical results.

==> pmi-body-elevator.tex <==



 \section{Case Study}   \label{sec:elevator}
 We illustrate the application of concepts in the previous sections through an elevator example inspired by  \cite{Hong:1997}.  An elevator is a real-time system, has control loops, is a SoS, and its operation is commonly understood. Consider an elevator system with 5 floors, and physical components such as doors, motor, and elevator car.  We describe the elevator system first, followed by the representation of two effects. Unfortunately, the length limit of this paper does not allow us to present full details of the elevator system, which is available separately \cite{damodaran2018elevator}.
 \subsection{Elevator System}
 Figure \ref{fig:elevator-system} specifies the model of this elevator. Table \ref{table:Elevator} describes each component of this model and its function.   
 
% \begin{table}[h]
%    \centering
%    \small
%    \caption{Elevator component-functionality map}
%    \begin{tabular}{ | l | l | p{12cm} |}
%    \hline
%    \textbf{ID} & \textbf{Name} & \textbf{Function} \\ \hline
%    F1 & ElevatorCtrl & Implements the control logic for elevator movement \\ \hline
%    F2 & RequestProc & Collects and forwards inputs such as destination floor requests from different floors and inside the car to F1\\ \hline
%    F3 & DoorStatusProc & Provides the door status of both the floor and the car door to ElevatorCtrl(F1) \\ \hline
%    F4 & Car & This is the elevator car that moves between the floors \\ \hline
%    F4.1 & Motor & A motor that activates the pulley for the Car (F4) \\ \hline
%    F4.2 & CarCtrl & \textit{controller} that operates motor and car door under commands from ElevatorCtrl, and provides car position to ElevatorCtrl(F1)\\ \hline
%    F4.3 & CarBtn & Button inside the car that generates a floor request to RequestProc(F2)\\ \hline
%    F4.4 & CarDoor & Car door  position sensor, sends position to DoorStatusProc(F3)\\ \hline
%    F5 & Floor & Floors 1-5  with a floor button to send requests to RequestProc(F2) and a floor door\\ \hline
%  \end{tabular}
%  \label{table:Elevator}
%\end{table}

 \setlength\LTleft{0pt}
\setlength\LTright{0pt} 
\small
    \begin{longtable}[h]{ | l | l | p{8cm} |}
    \hline
    \textbf{ID} & \textbf{Name} & \textbf{Function} \\ \hline
    F1 & ElevatorCtrl & Implements the control logic for elevator movement \\ \hline
    F2 & RequestProc & Collects and forwards inputs such as destination floor requests from different floors and inside the car to F1\\ \hline
    F3 & DoorStatusProc & Provides the door status of both the floor and the car door to ElevatorCtrl(F1) \\ \hline
    F4 & Car & This is the elevator car that moves between the floors \\ \hline
    F4.1 & Motor & A motor that activates the pulley for the Car (F4) \\ \hline
    F4.2 & CarCtrl & \textit{controller} that operates motor and car door under commands from ElevatorCtrl, and provides car position to ElevatorCtrl(F1)\\ \hline
    F4.3 & CarBtn & Button inside the car that generates a floor request to RequestProc(F2)\\ \hline
    F4.4 & CarDoor & Car door  position sensor, sends position to DoorStatusProc(F3)\\ \hline
    F5 & Floor & Floors 1-5  with a floor button to send requests to RequestProc(F2) and a floor door\\ \hline
          \caption{Elevator component-functionality map}
        \label{table:Elevator}
  \end{longtable}
  \normalsize


The model described in Figure \ref{fig:elevator-system}  does not have physics models of pulleys, motors, and doors since our focus is limited to cyber effects on the control loop of the elevator (Figure \ref{fig:elevator-control-loop}). The floor model combines the floor button and the floor door.


\begin{figure}
\centering
\begin{minipage}{.9\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{elevator-system}
  \captionof{figure}{Elevator Model}
    \label{fig:elevator-system}
\end{minipage}%
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.9\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{elevator-control-loop}
  \captionof{figure}{Elevator Control Loop}
    \label{fig:elevator-control-loop}
\end{minipage}%
\end{figure}
\begin{wrapfigure}{r}{0.60\textwidth}
  \begin{center}
    \includegraphics[width=0.6\textwidth]{h5-injection-script}
  \end{center}
 \caption{H5 Attack Simulation Script}
    \label{fig:h5-injection-script}
\end{wrapfigure}
\subsection{Representation of Attack H5}
We describe a simple attack on the elevator for illustration purposes, using the approach described in Section \ref{sec:effect-representation}. First we describe the attack tree in Figure \ref{fig:h5-attack-tree}, followed by the state diagrams in the process models of the Elevator Controller, ($F1$), and Car Controller, ($F4.2$), described in Table \ref{table:Elevator} and Figure \ref{fig:elevator-control-loop}. We also provide an attack simulation script to precisely describe the effect. In addition, we also provide a sequence diagram that describes how the effects unfold when the script is executed.



The attack tree in Figure \ref{fig:h5-attack-tree} describes how an attacker gains access to the motor and then changes its inputs and outputs to create an effect of the elevator going to the wrong floor.  The attack originates at the Motor ($F4.1$) and the target of the attack is the Elevator Controller ($F1$). The attack simulator is inserted into the elevator system described in Figure \ref{fig:elevator-system} to intercept all communications among these components, directly and indirectly. We omit the rewired system diagram. The forced transitions that result from this attack are shown in the process model of the Car Controller in Figure \ref{fig:h5-car-controller} as a transition (moving, reached), and the process model of the Elevator Controller in Figure \ref{fig:h5-elevator-controller} as (movingUP, stopped). These are forced external transitions among known states, as defined in Definition \ref{def:process-model}.

Line 1 in the simulation script, as described in Figure \ref{fig:h5-injection-script}, defines effect H5\_0, which generates a new message with type MsgMotor between Motor and CarCtrl with the value of cmd=REACHED,  when the attack simulator receives a message sent from CarCtrl to Motor with cmd==FORWARD. Line 3 specifies effect H5\_1, which drops a message received with the same attributes as effect H5\_0. Line 5 specifies a chaining of effects H5\_0 and H5\_1 into H5. The result of the chaining is that the same message that was received as specified in H5\_0 is dropped in H5\_1. Note that the injection operator for drop operation is the same as the delay operator with an infinite delay, as explained in Section \ref{sec:injection-protocol}. Line 6 activates effect H5 when the attack simulator receives a MsgCar sent from Car Controller to Elevator Controller, saying the Car Controller is READYTOMOVE and when at floor 1 (pos==1), and the user presses Car Button ($F4.3$) for destination floor (dest==3). Deactivation of H5 is omitted. 

The sequence diagram in Figure \ref{fig:h5-sequence-diagram} describes how the effect plays out. The effect is activated when the user presses Car Button to go to floor 3 from floor 1.  The Attack Simulator component is able to apply effect H5 twice, thus making the forced transitions occur twice, resulting in the elevator car staying at floor 1, instead of moving to floor 3.


\begin{figure}
\centering
\begin{minipage}{.3\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{h5-attack-tree}
  \captionof{figure}{H5 Attack Tree}
    \label{fig:h5-attack-tree}
\end{minipage}%
\begin{minipage}{.7\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{h5-sequence-diagram}
  \captionof{figure}{H5 Sequence Diagram}
    \label{fig:h5-sequence-diagram}
\end{minipage}
\end{figure}

%\begin{wrapfigure}{r}{0.40\textwidth}
%  \begin{center}
%    \includegraphics[width=0.40\textwidth]{h5-attack-tree}
%  \end{center}
% \caption{H5 Attack Tree}
%    \label{fig:h5-attack-tree}
%\end{wrapfigure}
%
%\begin{wrapfigure}{r}{0.60\textwidth}
%  \begin{center}
%    \includegraphics[width=0.60\textwidth]{h5-sequence-diagram}
%  \end{center}
% \caption{H5 Sequence Diagram}
%    \label{fig:h5-sequence diagram}
%\end{wrapfigure}



\begin{figure}
\centering
\begin{minipage}{1.0\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{h5-car-controller}
  \captionof{figure}{H5 Car Controller}
    \label{fig:h5-car-controller}
\end{minipage}%
\end{figure}

\begin{figure}
\centering
\begin{minipage}{1.0\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{h5-elevator-controller}
  \captionof{figure}{H5 Elevator Controller}
    \label{fig:h5-elevator-controller}
\end{minipage}%
\end{figure}


\section{Conclusions}   \label{sec:conclusions}

This paper describes an approach to simulate attacks on CPS through the injection of cyber effects using an attack simulator. This attack simulator is inserted into the system or its LVC model. The effects are applied through a cyber effects injection protocol that includes conditional injection operators and their activation. The conditions include the state variable values of the process model of a model component, message variables that are communicated among the model components, and time. We defined the concept of process model inconsistency precisely, and show how it can be simulated using this protocol. 

In Section \ref{sec:introduction}, we outlined the requirements for simulation of cyber effects. Let us review how our efforts described in this paper measure up to these requirements for simulating the control loop impact of \textit{process model inconsistency}. The first requirement stipulates that no malware be used, and we do not use any malware in our approach. The second requirement stipulates that the approach should be applicable to a SoS.  We demonstrated the application of our approach to an elevator model that is a SoS in Section \ref{sec:elevator}. Through the use of DEVS formalism which supports hierarchical specification as the theoretical basis of our approach, our approach will remain applicable to SoS.  In practice, the algorithm for the insertion of the attack simulator that has been defined in \cite{damodaran2017controlled} needs to be extended to a SoS environment. We plan to report on this extended algorithm in the near future.  The third requirement asks for a precise representation of the effects so as to be able to automate it. We described how to represent effects  in Section \ref{sec:effect-representation}, and further demonstrated its use in the case study.  The representation of effects includes a precise description of the forced state transitions, and the precise description of cyber effects injection using the cyber effects injection protocol. We have not reported the automation of the injection of these effects in this paper, and we expect to report on the automation in a forthcoming paper. This paper did not provide examples of time-based effects. An important future work is to describe the implementation of  time-based effects. Reactive effects, where an effect is triggered based on the result of a previous effect, is an obvious extension of our work for the near future.

The techniques described in this paper are readily applicable to Live and Virtual models since these models expose their operationally relevant API that may be used to inject effects. When the virtual models have less fidelity, and have only exposed minimal operationally relevant API, for example, only the time taken to complete an operation, it is not possible to demonstrate attacks on these models. However, even attacks on such lower fidelity models may be simulated using other models with higher fidelity. For example, in Section \ref{sec:elevator}, we discussed the attack on the motor, though the motor itself did not have a high-fidelity model to apply the effect. Instead, we were able to simulate the impact of such an attack on the Car Controller. Investigation of how to simulate process model inconsistency impacts in constructive simulations is an interesting area for future research.

This paper also does not address how to evaluate mitigation techniques after the application of cyber effects, again, an area of future work. A method for  generation of cyber effects based on process model, and development of an effects algebra to prove sufficiency and applicability of the effects injection protocol, are also anticipated future works.

%Inconsistency introduces a separate problem in addition to potential reachability to a \textit{bad state}. This is the system recovery problem of how to achieve reachability  from a \textit{reached state} to a \textit{known state} that is also a \textit{normal state}. We do not discuss any further this problem in this paper.


\begin{acks}
This research was funded by The MITRE Corporation's independent research and development program.  We thank Gabriel Pascualy for help with creating the diagrams used in the case study, and Paul Rowe for helpful discussions and review. 
\end{acks}


\subsection{Copyright}
Copyright \copyright\ \volumeyear\ The MITRE Corporation
%SAGE Publications Ltd,
%1 Oliver's Yard, 55 City Road, London, EC1Y~1SP, UK. 
All
rights reserved.

